Modeling Color Terminology Across Thousands of Languages

There is an extensive history of scholarship into what constitutes a "basic" color term, as well as a broadly attested acquisition sequence of basic color terms across many languages, as articulated in the seminal work of Berlin and Kay (1969). This paper employs a set of diverse measures on massively cross-linguistic data to operationalize and critique the Berlin and Kay color term hypotheses. Collectively, the 14 empirically-grounded computational linguistic metrics we design---as well as their aggregation---correlate strongly with both the Berlin and Kay basic/secondary color term partition (gamma=0.96) and their hypothesized universal acquisition sequence. The measures and result provide further empirical evidence from computational linguistics in support of their claims, as well as additional nuance: they suggest treating the partition as a spectrum instead of a dichotomy.

==> figures/trie.tex <==
\begin{forest}
for tree={
  circle,
  black,
  draw,
  fill=blue!40,
}
  [{}
    [{}, edge label={node [midway, above left] {B}}
      [{}, edge label={node [midway, right] {A}}
        [{}, edge label={node [midway, right] {U}}
          [,phantom]
          [{}, edge label={node [midway, left] {E}}
            [{}, edge label={node [midway, left] {R}}, label=below:Bauer
            ]
            [,phantom]
          ]
          [{}, edge label={node [midway, right] {M}}, label=below:Baum
          ]
          [,phantom]
        ]
        [,phantom]
      ]
      [,phantom]
    ]
    [{}, edge label={node [midway, right] {F}}
      [{}, edge label={node [midway, right] {E}}
        [{}, edge label={node [midway, right] {L}}
          [{}, edge label={node [midway, right] {D}}, label=below:Feld
          ]
          [,phantom]
        ]
        [,phantom]
      ]
      [,phantom]
    ]
    [{}, edge label={node [midway, left] {H}}
      [{}, edge label={node [midway, left] {A}}
        [{}, edge label={node [midway, left] {H}}
          [{}, edge label={node [midway, left] {N}}, label=below:Hahn
          ]
          [,phantom]
        ]
        [{}, edge label={node [midway, right] {U}}
          [{}, edge label={node [midway, left] {S}}, label=below:Haus
          ]
          [,phantom]
        ]
        [,phantom]
      ]
      [{}, edge label={node [midway, left] {O}}
        [{}, edge label={node [midway, right] {F}}, label=below:Hof
        ]
      ]
      [{}, edge label={node [midway, right] {U}}
        [,phantom]
        [{}, edge label={node [midway, left] {H}}
          [{}, edge label={node [midway, right] {N}}, label=below:Huhn
          ]
        ]
        [{}, edge label={node [midway, right] {N}}
          [,phantom]
          [{}, edge label={node [midway, right] {D}}, label=below:Hund
          ]
        ]
      ]
    ]
    [{}, edge label={node [midway, above right] {K}}
      [,phantom]
      [{}, edge label={node [midway, right] {A}}
        [,phantom]
        [{}, edge label={node [midway, right] {T}}
          [,phantom]
          [{}, edge label={node [midway, right] {Z}}
            [,phantom]
            [{}, edge label={node [midway, right] {E}}, label=below:Katze
            ]
          ]
        ]
      ]
    ]
  ]
\end{forest}

